Structural Econometric Estimation of the Basic Reproduction Number for Covid-19 Across U.S. States and Selected Countries

This paper proposes a structural econometric approach to estimating the basic reproduction number ($\mathcal{R}_{0}$) of Covid-19. This approach identifies $\mathcal{R}_{0}$ in a panel regression model by filtering out the effects of mitigating factors on disease diffusion and is easy to implement. We apply the method to data from 48 contiguous U.S. states and a diverse set of countries. Our results reveal a notable concentration of $\mathcal{R}_{0}$ estimates with an average value of 4.5. Through a counterfactual analysis, we highlight a significant underestimation of the $\mathcal{R}_{0}$ when mitigating factors are not appropriately accounted for.

==> tables/country_summary_statistics_fullsample.tex <==
\begin{table}
\centering
\caption{Summary statistics by country for the full sample (ending November 30, 2021)}
{\footnotesize
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
{} & \multicolumn{2}{c}{Delta} & \multicolumn{2}{c}{Stringency} & \multicolumn{2}{c}{Support} & \multicolumn{2}{c}{Threshold Ind.} & \multicolumn{2}{c}{Vaccinated} \\
{} &  mean &    std &       mean &    std &    mean &    std & mean &    std & mean &    std \\
\midrule
\textbf{Argentina  } &  0.10 & (0.23) &       0.78 & (0.15) &    0.60 & (0.18) & 1.00 & (0.06) & 0.18 & (0.26) \\
\textbf{Australia  } &  0.31 & (0.43) &       0.63 & (0.12) &    0.41 & (0.35) & 1.00 & (0.00) & 0.13 & (0.22) \\
\textbf{Brazil     } &  0.17 & (0.34) &       0.64 & (0.12) &    0.27 & (0.20) & 0.99 & (0.12) & 0.17 & (0.26) \\
\textbf{Chile      } &  0.14 & (0.31) &       0.74 & (0.16) &    0.67 & (0.39) & 0.99 & (0.08) & 0.26 & (0.32) \\
\textbf{Colombia   } &  0.14 & (0.29) &       0.69 & (0.16) &    0.73 & (0.09) & 0.99 & (0.09) & 0.12 & (0.20) \\
\textbf{Ecuador    } &  0.15 & (0.31) &       0.67 & (0.13) &    0.74 & (0.08) & 0.98 & (0.15) & 0.14 & (0.24) \\
\textbf{Egypt      } &  0.21 & (0.39) &       0.58 & (0.18) &    0.72 & (0.13) & 0.99 & (0.10) & 0.02 & (0.05) \\
\textbf{France     } &  0.24 & (0.41) &       0.59 & (0.16) &    0.57 & (0.23) & 0.97 & (0.16) & 0.21 & (0.29) \\
\textbf{Germany    } &  0.25 & (0.41) &       0.62 & (0.16) &    0.40 & (0.12) & 0.99 & (0.10) & 0.21 & (0.28) \\
\textbf{Indonesia  } &  0.29 & (0.43) &       0.66 & (0.08) &    0.33 & (0.09) & 0.98 & (0.14) & 0.07 & (0.13) \\
\textbf{Japan      } &  0.21 & (0.39) &       0.43 & (0.08) &    0.92 & (0.20) & 0.99 & (0.10) & 0.15 & (0.27) \\
\textbf{Mexico     } &  0.24 & (0.40) &       0.60 & (0.17) &    0.26 & (0.27) & 0.99 & (0.11) & 0.13 & (0.19) \\
\textbf{Nigeria    } &  0.26 & (0.41) &       0.57 & (0.15) &    0.08 & (0.15) & 0.96 & (0.19) & 0.01 & (0.01) \\
\textbf{Peru       } &  0.13 & (0.29) &       0.77 & (0.12) &    0.60 & (0.14) & 0.99 & (0.10) & 0.10 & (0.18) \\
\textbf{Philippines} &  0.20 & (0.37) &       0.75 & (0.11) &    0.24 & (0.29) & 0.99 & (0.12) & 0.05 & (0.10) \\
\textbf{South Korea} &  0.23 & (0.39) &       0.54 & (0.09) &    0.44 & (0.12) & 0.99 & (0.10) & 0.15 & (0.26) \\
\textbf{Spain      } &  0.24 & (0.40) &       0.61 & (0.14) &    0.84 & (0.15) & 0.98 & (0.14) & 0.22 & (0.31) \\
\textbf{Thailand   } &  0.34 & (0.42) &       0.58 & (0.11) &    0.72 & (0.25) & 0.95 & (0.22) & 0.13 & (0.21) \\
\textbf{Turkey     } &  0.25 & (0.39) &       0.62 & (0.15) &    0.54 & (0.33) & 0.99 & (0.11) & 0.17 & (0.24) \\
\textbf{All        } &  0.21 & (0.38) &       0.64 & (0.16) &    0.53 & (0.31) & 0.98 & (0.12) & 0.14 & (0.24) \\
\bottomrule
\end{tabular}
}
\label{tab:country_summary_statistics_fullsample}
\end{table}


==> tables/country_summary_statistics_subsample.tex <==
\begin{table}
\centering
\caption{Summary statistics by country for the pre-vaccination sample (ending January 31, 2021)}
{\footnotesize
\begin{tabular}{l|cc|cc|cc}
\toprule
{} & \multicolumn{2}{c}{Stringency} & \multicolumn{2}{c}{Support} & \multicolumn{2}{c}{Threshold Ind.} \\
{} &       mean &    std &    mean &    std & mean &    std \\
\midrule
\textbf{Argentina  } &       0.86 & (0.11) &    0.72 & (0.15) & 0.99 & (0.08) \\
\textbf{Australia  } &       0.65 & (0.12) &    0.69 & (0.17) & 1.00 & (0.00) \\
\textbf{Brazil     } &       0.68 & (0.13) &    0.42 & (0.17) & 0.97 & (0.16) \\
\textbf{Chile      } &       0.79 & (0.15) &    0.71 & (0.31) & 0.99 & (0.11) \\
\textbf{Colombia   } &       0.76 & (0.13) &    0.72 & (0.12) & 0.98 & (0.12) \\
\textbf{Ecuador    } &       0.71 & (0.17) &    0.72 & (0.12) & 0.96 & (0.21) \\
\textbf{Egypt      } &       0.72 & (0.15) &    0.68 & (0.17) & 0.98 & (0.14) \\
\textbf{France     } &       0.64 & (0.17) &    0.68 & (0.24) & 0.97 & (0.17) \\
\textbf{Germany    } &       0.62 & (0.13) &    0.42 & (0.16) & 0.98 & (0.13) \\
\textbf{Indonesia  } &       0.63 & (0.09) &    0.28 & (0.10) & 0.96 & (0.19) \\
\textbf{Japan      } &       0.37 & (0.07) &    0.85 & (0.26) & 0.98 & (0.13) \\
\textbf{Mexico     } &       0.70 & (0.15) &    0.25 & (0.35) & 0.98 & (0.15) \\
\textbf{Nigeria    } &       0.68 & (0.14) &    0.15 & (0.19) & 0.93 & (0.26) \\
\textbf{Peru       } &       0.81 & (0.13) &    0.68 & (0.16) & 0.98 & (0.14) \\
\textbf{Philippines} &       0.76 & (0.15) &    0.42 & (0.28) & 0.97 & (0.17) \\
\textbf{South Korea} &       0.56 & (0.09) &    0.45 & (0.13) & 0.98 & (0.13) \\
\textbf{Spain      } &       0.66 & (0.15) &    0.81 & (0.21) & 0.98 & (0.13) \\
\textbf{Thailand   } &       0.60 & (0.16) &    0.81 & (0.39) & 0.84 & (0.37) \\
\textbf{Turkey     } &       0.64 & (0.12) &    0.75 & (0.26) & 0.97 & (0.16) \\
\textbf{All        } &       0.68 & (0.17) &    0.58 & (0.30) & 0.97 & (0.16) \\
\bottomrule
\end{tabular}
}
\label{tab:country_summary_statistics_subsample}
\end{table}


==> tables/international_no_mitigating_factors.tex <==

    \begin{table}[!hp]
    \caption{Estimates of $\mathcal{R}_0$ across 19 countries without mitigating factors}
    \centering 
    \begin{footnotesize}
    \begin{tabular}{lccccc}\toprule 
    &\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
    &\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
    \cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
    & MF & MF && MF& MF \\
    Country& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
    Australia&1.14 [0.09]&1.14 [0.09]&&1.04 [0.13]&1.04 [0.13]\\
Brazil&1.45 [0.07]&1.45 [0.07]&&1.54 [0.12]&1.54 [0.12]\\
Chile&1.38 [0.06]&1.38 [0.06]&&1.42 [0.09]&1.42 [0.09]\\
Colombia&1.37 [0.05]&1.37 [0.05]&&1.44 [0.06]&1.44 [0.06]\\
Ecuador&1.23 [0.08]&1.23 [0.08]&&1.39 [0.15]&1.39 [0.15]\\
Egypt&1.12 [0.05]&1.12 [0.05]&&1.22 [0.08]&1.22 [0.08]\\
France&1.69 [0.17]&1.69 [0.17]&&1.55 [0.18]&1.55 [0.18]\\
Germany&1.36 [0.10]&1.36 [0.10]&&1.41 [0.14]&1.41 [0.14]\\
Indonesia&1.12 [0.06]&1.12 [0.06]&&1.34 [0.07]&1.34 [0.07]\\
Japan&1.09 [0.07]&1.09 [0.07]&&1.26 [0.08]&1.26 [0.08]\\
Mexico&1.20 [0.06]&1.20 [0.06]&&1.38 [0.08]&1.38 [0.08]\\
Nigeria&1.07 [0.06]&1.07 [0.06]&&1.25 [0.08]&1.25 [0.08]\\
Peru&1.35 [0.07]&1.35 [0.07]&&1.47 [0.11]&1.47 [0.11]\\
Philippines&1.17 [0.06]&1.17 [0.06]&&1.27 [0.09]&1.27 [0.09]\\
South Korea&1.10 [0.05]&1.10 [0.05]&&1.09 [0.09]&1.09 [0.09]\\
Spain&1.53 [0.12]&1.53 [0.12]&&1.59 [0.18]&1.59 [0.18]\\
Thailand&1.31 [0.14]&1.31 [0.14]&&1.59 [0.37]&1.59 [0.37]\\
Turkey&1.43 [0.12]&1.43 [0.12]&&1.46 [0.22]&1.46 [0.22]\\
    \bottomrule\end{tabular}
    \end{footnotesize}
    \begin{tablenotes}
    \scriptsize
    \item
    Notes: Numbers in brackets are standard errors robust to serial correlation and cross-sectional correlation (robust2). The multiplication factor (MF) declines linearly from the high value to the low value.
    \end{tablenotes}
    \label{tab:county_R0_no_mit}
    \end{table}
    

==> tables/lit_summary.tex <==
\begin{table}[thb!]
    \centering
    \caption{Reported $\mathcal{R}_0$ estimates for Covid-19 from selected studies}
    \renewcommand{\arraystretch}{1.2}
    {\footnotesize
    \begin{tabular}{p{0.2\textwidth}P{0.15\textwidth}P{0.21\textwidth}P{0.39\textwidth}}
    \toprule
        Study & Locations & Methods & $\mathcal{R}_0$ estimates \\
        \midrule
        \cite{Arias2023} & Belgium & SIRD model, MCMC & Slightly above 4 \\
        \cite{Buckman2020} & Brazil, China, Italy, US & SEIR model & Range from 4.8 to 11.4 (US=9.7) \\
        \cite{Chudik2022} & 9 Euro countries & Structural econometric approach & Range from 5.01 to 5.51 \\
        \cite{FernandezVillaverde2022} & Various cities, states, countries & SIRD model & Range from 1.5 to 2.4 (US=2.02) \\
        \cite{Katul2020} & 57 countries & SIR model & 4.5 \\
        \cite{Ke2021} & US and 8 Euro countries & SEIR model & Range from 3.6 and 6.4 (US=5.9 [4.7--7.5]) \\
        \cite{Korolev2021} & California, Japan, US & SEIRD model & Range from 1.69 to 19.55 \\
        \cite{Li2020} & China & Statistical exponential growth model & 2.2 [1.4--3.9] \\
        \cite{Liu2020a} & China & Statistical exponential growth model & 2.90 [2.32--3.63] \\
        & & Statistical maximum likelihood estimation & 2.92 [2.28--3.67] \\
        \cite{Locatelli2021} & 15 Euro countries & Statistical exponential growth model & 2.2 [1.9--2.6] \\
        \cite{Sanche2020} & China & Statistical exponential growth model & 5.7 [3.8--8.9] \\
        \cite{Wu2020} & China & SEIR model, MCMC & 2.68 [2.47--2.86] \\
        \cite{Zhao2020} & China & Statistical exponential growth model & Range from 2.24 [1.96--2.55] to 3.58 [2.89--4.39] \\
     \bottomrule
    \end{tabular}
    }
    \label{tab:lit_summary}  
    \vspace{-0.2cm}\flushleft\footnotesize{Note: The 95\% confidence intervals are in brackets.} 
\end{table}

==> tables/single_threshold_allsample_int_2023-05-08.tex <==
\begin{table}[!t]\caption{Estimation results for the mitigating factors across 19 countries}\centering 
\begin{small}
\begin{tabular}{lccccc}\toprule 
&\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
&\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
\cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
& MF & MF && MF& MF \\
Country& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
\bf Stringency Index&-1.68&-1.71&&-1.04&-1.07\\ 
standard s.e. (t-ratio)&0.14 (-11.8)&0.14 (-11.9)&&0.09 (-11.1)&0.10 (-10.8)\\ 
robust1 s.e. (t-ratio)&0.26 (-6.5)&0.26 (-6.7)&&0.19 (-5.6)&0.19 (-5.7)\\ 
robust2 s.e. (t-ratio)&0.35 (-4.7)&0.35 (-4.9)&&0.32 (-3.2)&0.31 (-3.4)\\ \midrule 
\bf Economic Support&-1.03&-1.01&&-0.61&-0.63\\ 
standard s.e. (t-ratio)&0.09 (-11.9)&0.09 (-11.6)&&0.05 (-11.1)&0.06 (-10.8)\\ 
robust1 s.e. (t-ratio)&0.13 (-7.8)&0.13 (-7.7)&&0.09 (-6.4)&0.09 (-6.6)\\ 
robust2 s.e. (t-ratio)&0.15 (-6.8)&0.15 (-6.8)&&0.14 (-4.4)&0.13 (-4.7)\\ \midrule 
\bf Vaccinated Share&&&&-0.78&-0.62\\ 
standard s.e. (t-ratio)&-&-&&0.09 (-8.6)&0.09 (-6.6)\\ 
robust1 s.e. (t-ratio)&-&-&&0.12 (-6.6)&0.12 (-5.0)\\ 
robust2 s.e. (t-ratio)&-&-&&0.18 (-4.3)&0.19 (-3.4)\\ \midrule 
\bf Delta Variant Share&&&&0.12&0.07\\ 
standard s.e. (t-ratio)&-&-&&0.06 (2.2)&0.06 (1.2)\\ 
robust1 s.e. (t-ratio)&-&-&&0.07 (1.7)&0.08 (1.0)\\ 
robust2 s.e. (t-ratio)&-&-&&0.12 (1.0)&0.12 (0.6)\\ \midrule 
\bf Threshold Indicator&-1.44&-1.42&&-1.81&-1.79\\ 
standard s.e. (t-ratio)&0.12 (-12.2)&0.12 (-11.9)&&0.09 (-19.1)&0.10 (-18.0)\\ 
robust1 s.e. (t-ratio)&0.31 (-4.7)&0.30 (-4.7)&&0.32 (-5.6)&0.32 (-5.6)\\ 
robust2 s.e. (t-ratio)&0.24 (-6.0)&0.24 (-5.9)&&0.35 (-5.2)&0.34 (-5.2)\\ \midrule 
Threshold Value&0.01&0.01&&0.01&0.01\\ 
R-squared&0.13&0.13&&0.09&0.08\\ 
\bottomrule\end{tabular}
\end{small}
\begin{tablenotes}
    \footnotesize
    \item
    Notes: The pre-vaccination sample includes 5,928 observations for 19 countries, covering a time span of $T_{\min}=140$  to $T_{\max}=329$  days. The full sample comprises 11,661 observations for the same 19 countries, spanning $T_{\min}=443$  to $T_{\max}=632$  days. Both estimation samples are unbalanced at the beginning. 
    ``Robust1" standard errors are robust to serial correlation only (Newey-West type correction), whereas ``robust2" standard errors are robust to serial correlation as well as any cross-sectional correlation. 
    Figures in parentheses are t-ratios. Oxford stringency and economic support indices are divided by 100 so that they take values between zero and one.
    Lag order is set to $p$ = 10 days in all regressions. The multiplication factor (MF) declines linearly from the high value to the low value.
\end{tablenotes}
\label{tab:country_regressors}
\end{table}

==> tables/single_threshold_allsample_intercept_int_2023-05-08.tex <==
\begin{table}[!t]\caption{Estimates of $\mathcal{R}_0$ across 19 countries}
\centering 
\resizebox{12cm}{!}{
\begin{tabular}{lccccc}\toprule 
&\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
&\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
\cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
& MF & MF && MF& MF \\
Country& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
Argentina&5.01 [0.51]&5.04 [0.50]&&4.41 [0.61]&4.51 [0.59]\\ 
Australia&4.27 [0.49]&4.26 [0.48]&&3.92 [0.59]&3.92 [0.57]\\ 
Brazil&4.47 [0.45]&4.52 [0.44]&&4.08 [0.56]&4.17 [0.54]\\ 
Chile&4.85 [0.48]&4.90 [0.47]&&4.46 [0.61]&4.53 [0.59]\\ 
Colombia&4.83 [0.46]&4.86 [0.45]&&4.32 [0.57]&4.41 [0.55]\\ 
Ecuador&4.69 [0.48]&4.70 [0.48]&&4.22 [0.59]&4.24 [0.57]\\ 
Egypt&4.54 [0.41]&4.53 [0.41]&&3.95 [0.53]&3.97 [0.51]\\ 
France&4.58 [0.45]&4.61 [0.44]&&4.35 [0.57]&4.47 [0.55]\\ 
Germany&4.18 [0.44]&4.19 [0.43]&&4.08 [0.58]&4.11 [0.56]\\ 
Indonesia&4.08 [0.40]&4.08 [0.39]&&3.80 [0.54]&3.82 [0.52]\\ 
Japan&4.16 [0.36]&4.14 [0.36]&&3.97 [0.52]&3.97 [0.50]\\ 
Mexico&4.21 [0.40]&4.22 [0.40]&&3.83 [0.52]&3.85 [0.50]\\ 
Nigeria&3.88 [0.40]&3.88 [0.40]&&3.42 [0.49]&3.44 [0.48]\\ 
Peru&4.89 [0.45]&4.93 [0.45]&&4.31 [0.59]&4.38 [0.56]\\ 
Philippines&4.37 [0.43]&4.38 [0.42]&&3.88 [0.56]&3.90 [0.54]\\ 
South Korea&3.85 [0.37]&3.84 [0.37]&&3.78 [0.51]&3.77 [0.49]\\ 
Spain&4.83 [0.49]&4.87 [0.48]&&4.44 [0.61]&4.56 [0.58]\\ 
Thailand&4.64 [0.54]&4.63 [0.53]&&4.12 [0.57]&4.14 [0.55]\\ 
Turkey&4.69 [0.52]&4.70 [0.51]&&4.22 [0.60]&4.28 [0.58]\\ 
\bottomrule\end{tabular}}
\begin{tablenotes}
\footnotesize
\item
Notes: The pre-vaccination sample includes 5,928 observations for 19 countries, covering a time span of $T_{\min}=140$  to $T_{\max}=329$  days. The full sample comprises 11,661 observations for the same 19 countries, spanning $T_{\min}=443$  to $T_{\max}=632$  days. Both estimation samples are unbalanced at the beginning. Numbers in brackets are standard errors robust to serial correlation and cross-sectional correlation (robust2). The multiplication factor declines linearly from the high value to the low value. The estimates on the mitigating factors are provided in Table \ref{tab:country_regressors} in the online supplement.
\end{tablenotes}
\label{tab:country_R0}
\end{table}

==> tables/single_threshold_allsample_intercept_states_2023-05-08.tex <==
\begin{table}[!hp]
\caption{Estimates of $\mathcal{R}_0$ across 48 contiguous U.S. states}
\centering 
\vspace{-0.3cm}
\begin{footnotesize}
\begin{tabular}{lccccc}\toprule 
&\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
&\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
\cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
& MF & MF && MF& MF \\
State& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
Alabama&4.29 [0.92]&4.60 [0.86]&&4.45 [0.81]&4.68 [0.76]\\ 
Arizona&4.62 [0.98]&4.92 [0.90]&&4.70 [0.83]&4.94 [0.78]\\ 
Arkansas&4.35 [0.97]&4.66 [0.90]&&4.50 [0.83]&4.76 [0.79]\\ 
California&4.77 [0.97]&5.08 [0.88]&&4.94 [0.90]&5.11 [0.87]\\ 
Colorado&4.62 [0.96]&4.92 [0.87]&&4.67 [0.85]&4.79 [0.80]\\ 
Connecticut&4.82 [1.02]&5.13 [0.92]&&4.79 [0.87]&4.91 [0.82]\\ 
Delaware&4.72 [1.01]&5.04 [0.92]&&4.75 [0.87]&4.93 [0.81]\\
District of Columbia&4.74 [1.09]&5.04 [0.98]&&4.68 [0.89]&4.77 [0.84]\\ 
Florida&4.41 [0.97]&4.73 [0.89]&&4.53 [0.83]&4.74 [0.78]\\ 
Georgia&4.41 [0.96]&4.76 [0.88]&&4.48 [0.83]&4.70 [0.78]\\ 
Idaho&4.36 [1.03]&4.63 [0.95]&&4.54 [0.85]&4.77 [0.80]\\ 
Illinois&4.68 [0.98]&5.00 [0.89]&&4.72 [0.84]&4.90 [0.79]\\ 
Indiana&4.34 [0.94]&4.66 [0.87]&&4.53 [0.84]&4.76 [0.79]\\ 
Iowa&4.29 [0.84]&4.73 [0.79]&&4.53 [0.80]&4.78 [0.76]\\ 
Kansas&4.65 [1.00]&4.95 [0.92]&&4.69 [0.84]&4.88 [0.79]\\ 
Kentucky&4.72 [1.06]&5.01 [0.96]&&4.73 [0.87]&4.92 [0.82]\\ 
Louisiana&4.70 [1.03]&5.01 [0.94]&&4.73 [0.89]&4.97 [0.84]\\ 
Maine&4.67 [1.15]&4.91 [1.04]&&4.71 [0.91]&4.74 [0.86]\\ 
Maryland&4.68 [1.01]&4.98 [0.92]&&4.66 [0.86]&4.73 [0.81]\\ 
Massachusetts&4.60 [1.05]&4.85 [0.96]&&4.79 [0.90]&4.95 [0.84]\\ 
Michigan&4.56 [1.05]&4.82 [0.96]&&4.71 [0.88]&4.86 [0.83]\\
Minnesota&4.57 [1.03]&4.85 [0.94]&&4.77 [0.87]&4.94 [0.82]\\ 
Mississippi&4.34 [0.95]&4.67 [0.89]&&4.44 [0.82]&4.67 [0.77]\\
Missouri&4.26 [0.94]&4.53 [0.87]&&4.46 [0.82]&4.64 [0.77]\\ 
Montana&4.27 [0.99]&4.58 [0.92]&&4.55 [0.84]&4.77 [0.79]\\ 
Nebraska&4.35 [0.96]&4.71 [0.89]&&4.51 [0.82]&4.77 [0.77]\\
Nevada&4.39 [1.01]&4.69 [0.93]&&4.55 [0.86]&4.78 [0.81]\\ 
New Hampshire&4.23 [0.96]&4.47 [0.89]&&4.49 [0.85]&4.56 [0.80]\\ 
New Jersey&4.73 [0.98]&5.07 [0.89]&&4.75 [0.85]&4.91 [0.80]\\ 
New Mexico&4.79 [1.23]&5.07 [1.11]&&4.87 [0.94]&5.06 [0.88]\\ 
New York&4.85 [1.01]&5.18 [0.91]&&4.66 [0.87]&4.70 [0.82]\\ 
North Carolina&4.69 [1.04]&4.96 [0.95]&&4.66 [0.87]&4.81 [0.82]\\ 
North Dakota&4.24 [0.89]&4.68 [0.84]&&4.67 [0.80]&5.17 [0.76]\\ 
Ohio&4.41 [1.05]&4.66 [0.96]&&4.56 [0.87]&4.72 [0.81]\\ 
Oklahoma&4.21 [0.87]&4.50 [0.82]&&4.48 [0.82]&4.72 [0.77]\\ 
Oregon&4.55 [0.97]&4.82 [0.89]&&4.60 [0.86]&4.62 [0.81]\\ 
Pennsylvania&4.64 [0.98]&4.92 [0.90]&&4.65 [0.84]&4.75 [0.79]\\ 
Rhode Island&4.88 [1.01]&5.29 [0.92]&&4.95 [0.88]&5.26 [0.83]\\ 
South Carolina&4.32 [0.92]&4.64 [0.85]&&4.51 [0.82]&4.75 [0.77]\\ 
South Dakota&4.25 [0.88]&4.65 [0.83]&&4.64 [0.81]&5.05 [0.76]\\ 
Tennessee&4.43 [1.03]&4.73 [0.95]&&4.59 [0.85]&4.92 [0.80]\\ 
Texas&4.45 [1.01]&4.73 [0.93]&&4.54 [0.85]&4.73 [0.80]\\ 
Utah&4.33 [0.96]&4.65 [0.89]&&4.55 [0.82]&4.87 [0.77]\\ 
Vermont&4.23 [1.05]&4.59 [0.97]&&4.45 [0.88]&4.47 [0.83]\\ 
Virginia&4.36 [0.98]&4.64 [0.91]&&4.48 [0.85]&4.59 [0.80]\\ 
Washington&4.65 [0.99]&4.94 [0.91]&&4.64 [0.88]&4.68 [0.83]\\ 
Wisconsin&4.57 [0.96]&4.89 [0.88]&&4.76 [0.85]&4.99 [0.80]\\ 
Wyoming&4.55 [1.02]&4.77 [0.94]&&4.58 [0.84]&4.69 [0.79]\\ 
\bottomrule\end{tabular}
\end{footnotesize}
\begin{tablenotes}
\scriptsize
\item
Notes: The pre-vaccination sample includes 14,996 observations for $N=48$ states, covering a time span of $T_{\min}=163$ to $T_{\max}=331$ days. The full sample comprises 29,531 observations, spanning $T_{\min}=457$  to $T_{\max}=634$  days. Both estimation samples are unbalanced at the beginning. Numbers in brackets are standard errors robust to serial correlation and cross-sectional correlation (robust2). The multiplication factor (MF) declines linearly from the high value to the low value. The estimates on the mitigating factors are provided in Table \ref{tab:state_regressors} in the online supplement.
\end{tablenotes}
\label{tab:state_R0}
\end{table}

==> tables/single_threshold_allsample_states_2023-05-08.tex <==
\begin{table}[!th]\caption{Estimation results for the mitigating factors across 48 contiguous U.S. states}\centering 
\begin{small}
\begin{tabular}{lccccc}\toprule 
&\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
&\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
\cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
& MF & MF && MF& MF \\
State& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
\bf Stringency Index&-1.28&-1.27&&-1.07&-1.51\\ 
standard s.e. (t-ratio)&0.08 (-15.4)&0.09 (-14.5)&&0.11 (-9.6)&0.13 (-11.5)\\ 
robust1 s.e. (t-ratio)&0.15 (-8.7)&0.14 (-9.1)&&0.14 (-7.7)&0.15 (-9.8)\\ 
robust2 s.e. (t-ratio)&1.16 (-1.1)&0.97 (-1.3)&&0.64 (-1.7)&0.60 (-2.5)\\ \midrule 
\bf Economic Support&-0.39&-0.63&&-0.03&0.02\\ 
standard s.e. (t-ratio)&0.06 (-6.3)&0.06 (-9.9)&&0.07 (-0.4)&0.09 (0.3)\\ 
robust1 s.e. (t-ratio)&0.12 (-3.2)&0.12 (-5.2)&&0.09 (-0.3)&0.10 (0.2)\\ 
robust2 s.e. (t-ratio)&0.32 (-1.2)&0.33 (-1.9)&&0.20 (-0.1)&0.23 (0.1)\\ \midrule 
\bf Vaccinated Share&&&&-1.65&-1.51\\ 
standard s.e. (t-ratio)&-&-&&0.10 (-17.2)&0.11 (-13.3)\\ 
robust1 s.e. (t-ratio)&-&-&&0.08 (-19.8)&0.10 (-15.2)\\ 
robust2 s.e. (t-ratio)&-&-&&0.40 (-4.2)&0.44 (-3.4)\\ \midrule 
\bf Delta Variant Share&&&&1.00&1.00\\ 
standard s.e. (t-ratio)&-&-&&0.04 (22.8)&0.05 (19.4)\\ 
robust1 s.e. (t-ratio)&-&-&&0.04 (24.7)&0.05 (18.9)\\ 
robust2 s.e. (t-ratio)&-&-&&0.18 (5.5)&0.24 (4.1)\\ \midrule 
\bf Rep $\times$ Economic Support&0.42&0.39&&0.26&0.18\\ 
standard s.e. (t-ratio)&0.07 (6.1)&0.07 (5.4)&&0.09 (3.0)&0.10 (1.8)\\ 
robust1 s.e. (t-ratio)&0.15 (2.8)&0.14 (2.7)&&0.10 (2.7)&0.11 (1.7)\\ 
robust2 s.e. (t-ratio)&0.14 (3.0)&0.14 (2.7)&&0.09 (2.8)&0.10 (1.8)\\ \midrule 
\bf Threshold Indicator&-2.31&-2.37&&-2.71&-2.49\\ 
standard s.e. (t-ratio)&0.04 (-62.2)&0.04 (-54.6)&&0.07 (-39.1)&0.08 (-30.6)\\ 
robust1 s.e. (t-ratio)&0.11 (-20.3)&0.12 (-19.1)&&0.13 (-20.7)&0.13 (-19.3)\\ 
robust2 s.e. (t-ratio)&0.50 (-4.6)&0.53 (-4.5)&&0.59 (-4.6)&0.55 (-4.5)\\ \midrule 
Threshold Value&0.70&0.40&&0.40&0.40\\ 
R-squared&0.31&0.29&&0.09&0.08\\ 
\bottomrule\end{tabular}
\end{small}
\begin{tablenotes}
\footnotesize
\item
Notes: The pre-vaccination sample includes 14,996 observations for 48 contiguous states, covering a time span of $T_{\min}=163$ to $T_{\max}=331$ days. The full sample comprises 29,531 observations, spanning $T_{\min}=457$  to $T_{\max}=634$ days. Both estimation samples are unbalanced at the beginning.
Rep is a dummy variable equal to one for a Republican governor.
``Robust1" standard errors are robust to serial correlation only (Newey-West type correction), whereas ``robust2" standard errors are robust to serial correlation as well as any cross-sectional correlation. 
Figures in parentheses are t-ratios. Oxford stringency and economic support indices are divided by 100 so that they take values between zero and one.
Lag order is set to $p$ = 10 days in all regressions. The multiplication factor (MF) declines linearly from the high value to the low value.
\end{tablenotes}
\label{tab:state_regressors}
\end{table}

==> tables/state_summary_statistics_fullsample.tex <==
\begin{table}
\centering
\caption{Summary statistics by state for the full sample (ending November 30, 2021)}
{\footnotesize
\begin{tabular}{l|cc|cc|cc|cc|cc|}
\toprule
{} & \multicolumn{2}{c}{delta} & \multicolumn{2}{c}{stringency} & \multicolumn{2}{c}{support} & \multicolumn{2}{c}{thr} & \multicolumn{2}{c}{vaxx} \\
{} &  mean &    std &       mean &    std &    mean &    std & mean &    std & mean &    std \\
\midrule
\textbf{Alabama             } &  0.26 & (0.41) &       0.43 & (0.13) &    0.39 & (0.14) & 0.98 & (0.13) & 0.13 & (0.17) \\
\textbf{Arizona             } &  0.25 & (0.41) &       0.46 & (0.16) &    0.41 & (0.12) & 0.98 & (0.13) & 0.17 & (0.21) \\
\textbf{Arkansas            } &  0.28 & (0.43) &       0.48 & (0.13) &    0.41 & (0.15) & 0.99 & (0.11) & 0.14 & (0.18) \\
\textbf{California          } &  0.26 & (0.41) &       0.55 & (0.17) &    0.67 & (0.12) & 0.96 & (0.19) & 0.19 & (0.24) \\
\textbf{Colorado            } &  0.27 & (0.42) &       0.52 & (0.16) &    0.55 & (0.24) & 0.98 & (0.13) & 0.20 & (0.25) \\
\textbf{Connecticut         } &  0.25 & (0.41) &       0.55 & (0.19) &    0.67 & (0.21) & 0.98 & (0.13) & 0.23 & (0.29) \\
\textbf{Delaware            } &  0.25 & (0.41) &       0.55 & (0.16) &    0.62 & (0.17) & 0.99 & (0.09) & 0.19 & (0.24) \\
\textbf{District of Columbia} &  0.24 & (0.41) &       0.59 & (0.17) &    0.65 & (0.15) & 1.00 & (0.07) & 0.20 & (0.25) \\
\textbf{Florida             } &  0.24 & (0.41) &       0.46 & (0.20) &    0.44 & (0.27) & 0.98 & (0.15) & 0.18 & (0.23) \\
\textbf{Georgia             } &  0.25 & (0.41) &       0.50 & (0.16) &    0.49 & (0.29) & 0.98 & (0.15) & 0.14 & (0.18) \\
\textbf{Idaho               } &  0.24 & (0.41) &       0.49 & (0.16) &    0.39 & (0.16) & 0.99 & (0.12) & 0.14 & (0.18) \\
\textbf{Illinois            } &  0.25 & (0.42) &       0.51 & (0.18) &    0.59 & (0.18) & 0.98 & (0.14) & 0.18 & (0.23) \\
\textbf{Indiana             } &  0.26 & (0.42) &       0.48 & (0.14) &    0.47 & (0.22) & 0.98 & (0.14) & 0.16 & (0.20) \\
\textbf{Iowa                } &  0.27 & (0.42) &       0.43 & (0.14) &    0.58 & (0.28) & 0.99 & (0.12) & 0.19 & (0.23) \\
\textbf{Kansas              } &  0.28 & (0.43) &       0.49 & (0.15) &    0.53 & (0.18) & 0.99 & (0.12) & 0.17 & (0.21) \\
\textbf{Kentucky            } &  0.24 & (0.41) &       0.56 & (0.18) &    0.48 & (0.22) & 0.98 & (0.13) & 0.17 & (0.21) \\
\textbf{Louisiana           } &  0.24 & (0.41) &       0.58 & (0.10) &    0.42 & (0.20) & 0.98 & (0.13) & 0.15 & (0.18) \\
\textbf{Maine               } &  0.23 & (0.41) &       0.58 & (0.21) &    0.49 & (0.21) & 1.00 & (0.07) & 0.23 & (0.29) \\
\textbf{Maryland            } &  0.24 & (0.41) &       0.54 & (0.19) &    0.64 & (0.21) & 0.98 & (0.14) & 0.21 & (0.27) \\
\textbf{Massachusetts       } &  0.25 & (0.41) &       0.56 & (0.16) &    0.37 & (0.18) & 0.98 & (0.15) & 0.22 & (0.29) \\
\textbf{Michigan            } &  0.24 & (0.41) &       0.53 & (0.19) &    0.40 & (0.14) & 0.98 & (0.14) & 0.17 & (0.22) \\
\textbf{Minnesota           } &  0.25 & (0.42) &       0.51 & (0.17) &    0.37 & (0.18) & 0.98 & (0.13) & 0.20 & (0.25) \\
\textbf{Mississippi         } &  0.27 & (0.42) &       0.46 & (0.16) &    0.43 & (0.19) & 0.99 & (0.12) & 0.13 & (0.17) \\
\textbf{Missouri            } &  0.29 & (0.44) &       0.45 & (0.14) &    0.40 & (0.15) & 0.98 & (0.14) & 0.16 & (0.20) \\
\textbf{Montana             } &  0.27 & (0.42) &       0.45 & (0.14) &    0.39 & (0.15) & 0.99 & (0.12) & 0.19 & (0.21) \\
\textbf{Nebraska            } &  0.27 & (0.43) &       0.46 & (0.15) &    0.64 & (0.22) & 0.98 & (0.14) & 0.19 & (0.23) \\
\textbf{Nevada              } &  0.27 & (0.42) &       0.51 & (0.16) &    0.39 & (0.23) & 0.99 & (0.12) & 0.17 & (0.21) \\
\textbf{New Hampshire       } &  0.25 & (0.41) &       0.48 & (0.15) &    0.44 & (0.22) & 0.99 & (0.09) & 0.21 & (0.26) \\
\textbf{New Jersey          } &  0.26 & (0.42) &       0.51 & (0.17) &    0.66 & (0.15) & 0.98 & (0.13) & 0.21 & (0.27) \\
\textbf{New Mexico          } &  0.25 & (0.41) &       0.63 & (0.21) &    0.43 & (0.12) & 0.99 & (0.11) & 0.21 & (0.26) \\
\textbf{New York            } &  0.25 & (0.41) &       0.58 & (0.20) &    0.84 & (0.29) & 0.97 & (0.17) & 0.20 & (0.26) \\
\textbf{North Carolina      } &  0.25 & (0.41) &       0.56 & (0.16) &    0.50 & (0.22) & 0.98 & (0.15) & 0.16 & (0.20) \\
\textbf{North Dakota        } &  0.25 & (0.42) &       0.40 & (0.09) &    0.46 & (0.18) & 1.00 & (0.00) & 0.16 & (0.19) \\
\textbf{Ohio                } &  0.25 & (0.41) &       0.52 & (0.16) &    0.40 & (0.13) & 0.98 & (0.15) & 0.17 & (0.21) \\
\textbf{Oklahoma            } &  0.27 & (0.42) &       0.44 & (0.11) &    0.38 & (0.17) & 0.98 & (0.13) & 0.16 & (0.19) \\
\textbf{Oregon              } &  0.23 & (0.40) &       0.55 & (0.16) &    0.65 & (0.13) & 0.98 & (0.13) & 0.20 & (0.25) \\
\textbf{Pennsylvania        } &  0.25 & (0.42) &       0.49 & (0.18) &    0.56 & (0.16) & 0.98 & (0.14) & 0.19 & (0.24) \\
\textbf{Rhode Island        } &  0.25 & (0.41) &       0.57 & (0.17) &    0.70 & (0.19) & 1.00 & (0.07) & 0.23 & (0.28) \\
\textbf{South Carolina      } &  0.25 & (0.41) &       0.46 & (0.13) &    0.40 & (0.22) & 0.98 & (0.13) & 0.15 & (0.19) \\
\textbf{South Dakota        } &  0.27 & (0.43) &       0.40 & (0.11) &    0.39 & (0.13) & 1.00 & (0.06) & 0.19 & (0.22) \\
\textbf{Tennessee           } &  0.25 & (0.41) &       0.50 & (0.16) &    0.43 & (0.14) & 0.98 & (0.13) & 0.15 & (0.18) \\
\textbf{Texas               } &  0.25 & (0.41) &       0.49 & (0.13) &    0.41 & (0.13) & 0.98 & (0.15) & 0.16 & (0.21) \\
\textbf{Utah                } &  0.28 & (0.43) &       0.44 & (0.12) &    0.38 & (0.16) & 0.99 & (0.12) & 0.16 & (0.20) \\
\textbf{Vermont             } &  0.33 & (0.45) &       0.51 & (0.21) &    0.69 & (0.21) & 0.99 & (0.11) & 0.30 & (0.30) \\
\textbf{Virginia            } &  0.25 & (0.41) &       0.50 & (0.16) &    0.55 & (0.20) & 0.98 & (0.14) & 0.20 & (0.25) \\
\textbf{Washington          } &  0.25 & (0.41) &       0.57 & (0.17) &    0.69 & (0.20) & 0.98 & (0.13) & 0.20 & (0.26) \\
\textbf{West Virginia       } &  0.24 & (0.41) &       0.49 & (0.17) &    0.44 & (0.13) & 0.99 & (0.10) & 0.15 & (0.17) \\
\textbf{Wisconsin           } &  0.25 & (0.41) &       0.49 & (0.14) &    0.41 & (0.21) & 0.98 & (0.13) & 0.19 & (0.24) \\
\textbf{All                 } &  0.26 & (0.42) &       0.51 & (0.17) &    0.50 & (0.22) & 0.98 & (0.13) & 0.18 & (0.23) \\
\bottomrule
\end{tabular}
}
\label{tab:state_summary_statistics_fullsample}
\end{table}


==> tables/state_summary_statistics_subsample.tex <==
\begin{table}
\centering
\caption{Summary statistics by state for the pre-vaccination sample (ending January 31, 2021)}
{\footnotesize
\begin{tabular}{l|cc|cc|cc|cc|cc|}
\toprule
{} & \multicolumn{2}{c}{stringency} & \multicolumn{2}{c}{support} & \multicolumn{2}{c}{thr} \\
{} &       mean &    std &    mean &    std & mean &    std \\
\midrule
\textbf{Alabama             } &       0.52 & (0.12) &    0.43 & (0.18) & 0.97 & (0.18) \\
\textbf{Arizona             } &       0.58 & (0.07) &    0.47 & (0.14) & 0.97 & (0.18) \\
\textbf{Arkansas            } &       0.57 & (0.09) &    0.44 & (0.18) & 0.97 & (0.16) \\
\textbf{California          } &       0.65 & (0.12) &    0.70 & (0.16) & 0.93 & (0.25) \\
\textbf{Colorado            } &       0.62 & (0.12) &    0.70 & (0.18) & 0.97 & (0.18) \\
\textbf{Connecticut         } &       0.69 & (0.08) &    0.76 & (0.16) & 0.97 & (0.17) \\
\textbf{Delaware            } &       0.67 & (0.12) &    0.71 & (0.16) & 0.98 & (0.13) \\
\textbf{District of Columbia} &       0.73 & (0.08) &    0.68 & (0.18) & 0.99 & (0.10) \\
\textbf{Florida             } &       0.59 & (0.17) &    0.57 & (0.27) & 0.95 & (0.21) \\
\textbf{Georgia             } &       0.61 & (0.11) &    0.64 & (0.25) & 0.96 & (0.20) \\
\textbf{Idaho               } &       0.61 & (0.12) &    0.40 & (0.21) & 0.97 & (0.17) \\
\textbf{Illinois            } &       0.62 & (0.14) &    0.61 & (0.24) & 0.96 & (0.19) \\
\textbf{Indiana             } &       0.57 & (0.09) &    0.59 & (0.25) & 0.96 & (0.19) \\
\textbf{Iowa                } &       0.53 & (0.10) &    0.81 & (0.15) & 0.97 & (0.17) \\
\textbf{Kansas              } &       0.61 & (0.08) &    0.51 & (0.23) & 0.97 & (0.17) \\
\textbf{Kentucky            } &       0.69 & (0.11) &    0.61 & (0.25) & 0.97 & (0.18) \\
\textbf{Louisiana           } &       0.64 & (0.11) &    0.50 & (0.25) & 0.97 & (0.17) \\
\textbf{Maine               } &       0.76 & (0.12) &    0.60 & (0.24) & 0.99 & (0.10) \\
\textbf{Maryland            } &       0.67 & (0.15) &    0.68 & (0.19) & 0.96 & (0.19) \\
\textbf{Massachusetts       } &       0.64 & (0.11) &    0.42 & (0.19) & 0.96 & (0.20) \\
\textbf{Michigan            } &       0.64 & (0.15) &    0.44 & (0.17) & 0.96 & (0.19) \\
\textbf{Minnesota           } &       0.63 & (0.09) &    0.46 & (0.14) & 0.97 & (0.18) \\
\textbf{Mississippi         } &       0.56 & (0.13) &    0.48 & (0.24) & 0.97 & (0.16) \\
\textbf{Missouri            } &       0.53 & (0.12) &    0.42 & (0.18) & 0.97 & (0.18) \\
\textbf{Montana             } &       0.57 & (0.07) &    0.41 & (0.20) & 0.97 & (0.17) \\
\textbf{Nebraska            } &       0.59 & (0.10) &    0.58 & (0.15) & 0.97 & (0.16) \\
\textbf{Nevada              } &       0.61 & (0.09) &    0.50 & (0.23) & 0.97 & (0.17) \\
\textbf{New Hampshire       } &       0.57 & (0.16) &    0.50 & (0.29) & 0.98 & (0.13) \\
\textbf{New Jersey          } &       0.62 & (0.13) &    0.70 & (0.18) & 0.97 & (0.18) \\
\textbf{New Mexico          } &       0.81 & (0.04) &    0.48 & (0.12) & 0.98 & (0.15) \\
\textbf{New York            } &       0.72 & (0.11) &    0.95 & (0.22) & 0.95 & (0.23) \\
\textbf{North Carolina      } &       0.67 & (0.08) &    0.59 & (0.10) & 0.96 & (0.21) \\
\textbf{North Dakota        } &       0.47 & (0.05) &    0.41 & (0.20) & 1.00 & (0.00) \\
\textbf{Ohio                } &       0.64 & (0.09) &    0.46 & (0.15) & 0.96 & (0.21) \\
\textbf{Oklahoma            } &       0.47 & (0.14) &    0.39 & (0.21) & 0.97 & (0.18) \\
\textbf{Oregon              } &       0.64 & (0.09) &    0.71 & (0.16) & 0.97 & (0.18) \\
\textbf{Pennsylvania        } &       0.63 & (0.11) &    0.63 & (0.19) & 0.96 & (0.20) \\
\textbf{Rhode Island        } &       0.70 & (0.07) &    0.86 & (0.07) & 0.99 & (0.10) \\
\textbf{South Carolina      } &       0.54 & (0.11) &    0.51 & (0.19) & 0.97 & (0.18) \\
\textbf{South Dakota        } &       0.47 & (0.08) &    0.43 & (0.17) & 0.99 & (0.08) \\
\textbf{Tennessee           } &       0.61 & (0.09) &    0.42 & (0.19) & 0.97 & (0.18) \\
\textbf{Texas               } &       0.59 & (0.10) &    0.43 & (0.18) & 0.95 & (0.21) \\
\textbf{Utah                } &       0.54 & (0.07) &    0.39 & (0.21) & 0.97 & (0.17) \\
\textbf{Vermont             } &       0.69 & (0.09) &    0.67 & (0.17) & 0.96 & (0.19) \\
\textbf{Virginia            } &       0.61 & (0.10) &    0.57 & (0.21) & 0.96 & (0.20) \\
\textbf{Washington          } &       0.66 & (0.12) &    0.75 & (0.19) & 0.97 & (0.18) \\
\textbf{West Virginia       } &       0.62 & (0.09) &    0.49 & (0.14) & 0.98 & (0.14) \\
\textbf{Wisconsin           } &       0.58 & (0.11) &    0.52 & (0.21) & 0.97 & (0.18) \\
\textbf{All                 } &       0.62 & (0.13) &    0.56 & (0.24) & 0.97 & (0.18) \\
\bottomrule
\end{tabular}
}
\label{tab:state_summary_statistics_subsample}
\end{table}


==> tables/us_states_no_mitigating_factors.tex <==
\begin{table}[!hp]
\caption{Estimates of $\mathcal{R}_0$ across 48 contiguous U.S. states without mitigating factors}
\centering 
\begin{footnotesize}
\begin{tabular}{lccccc}\toprule 
&\multicolumn{2}{c}{\bf Pre-vaccination sample}&&\multicolumn{2}{c}{\bf Full sample} \\
&\multicolumn{2}{c}{\bf Ending Jan 31, 2021}&&\multicolumn{2}{c}{\bf Ending Nov 30, 2021} \\
\cline{2-3} \cline{3-3} \cline{5-6} \cline{6-6} 
& MF & MF && MF& MF \\
State& 5 to 2& 8 to 2.5 && 5 to 2 & 8 to 2.5 \\ \midrule
    Arizona&1.51 [0.07]&1.81 [0.08]&&1.48 [0.11]&1.61 [0.11]\\
Arkansas&1.45 [0.06]&1.73 [0.07]&&1.40 [0.07]&1.52 [0.07]\\
California&1.66 [0.32]&1.86 [0.37]&&1.53 [0.14]&1.60 [0.14]\\
Colorado&1.38 [0.07]&1.54 [0.07]&&1.34 [0.11]&1.41 [0.11]\\
Connecticut&1.38 [0.09]&1.54 [0.09]&&1.41 [0.13]&1.49 [0.13]\\
Delaware&1.39 [0.07]&1.60 [0.08]&&1.34 [0.09]&1.42 [0.09]\\
District of Columbia&1.25 [0.06]&1.35 [0.07]&&1.27 [0.09]&1.34 [0.09]\\
Florida&1.44 [0.09]&1.67 [0.09]&&1.48 [0.13]&1.58 [0.13]\\
Georgia&1.41 [0.08]&1.63 [0.09]&&1.46 [0.11]&1.56 [0.11]\\
Idaho&1.43 [0.07]&1.67 [0.08]&&1.36 [0.10]&1.47 [0.10]\\
Illinois&1.46 [0.09]&1.68 [0.09]&&1.45 [0.13]&1.56 [0.13]\\
Indiana&1.46 [0.08]&1.70 [0.09]&&1.42 [0.12]&1.52 [0.12]\\
Iowa&1.49 [0.07]&1.79 [0.08]&&1.42 [0.09]&1.56 [0.09]\\
Kansas&1.47 [0.06]&1.71 [0.07]&&1.44 [0.08]&1.55 [0.09]\\
Kentucky&1.42 [0.07]&1.63 [0.08]&&1.39 [0.08]&1.47 [0.08]\\
Louisiana&1.43 [0.09]&1.67 [0.10]&&1.47 [0.14]&1.59 [0.14]\\
Maine&1.22 [0.06]&1.27 [0.06]&&1.22 [0.07]&1.24 [0.07]\\
Maryland&1.30 [0.08]&1.41 [0.08]&&1.37 [0.11]&1.43 [0.11]\\
Massachusetts&1.41 [0.10]&1.59 [0.10]&&1.42 [0.14]&1.51 [0.14]\\
Michigan&1.43 [0.09]&1.60 [0.10]&&1.37 [0.13]&1.45 [0.13]\\
Minnesota&1.47 [0.08]&1.68 [0.09]&&1.39 [0.09]&1.48 [0.09]\\
Mississippi&1.42 [0.07]&1.67 [0.08]&&1.41 [0.09]&1.54 [0.09]\\
Missouri&1.45 [0.07]&1.66 [0.08]&&1.38 [0.10]&1.48 [0.10]\\
Montana&1.44 [0.06]&1.69 [0.07]&&1.36 [0.09]&1.47 [0.09]\\
Nebraska&1.47 [0.07]&1.75 [0.08]&&1.38 [0.09]&1.52 [0.09]\\
Nevada&1.42 [0.07]&1.65 [0.07]&&1.39 [0.10]&1.49 [0.10]\\
New Hampshire&1.29 [0.07]&1.38 [0.07]&&1.27 [0.08]&1.30 [0.08]\\
New Jersey&1.44 [0.10]&1.66 [0.11]&&1.46 [0.17]&1.56 [0.17]\\
New Mexico&1.40 [0.06]&1.58 [0.07]&&1.34 [0.08]&1.42 [0.09]\\
New York&1.30 [0.11]&1.37 [0.11]&&1.40 [0.18]&1.44 [0.17]\\
North Carolina&1.37 [0.07]&1.54 [0.07]&&1.41 [0.09]&1.48 [0.09]\\
North Dakota&1.62 [0.08]&2.17 [0.11]&&1.36 [0.07]&1.62 [0.08]\\
Ohio&1.40 [0.08]&1.57 [0.08]&&1.41 [0.11]&1.48 [0.11]\\
Oklahoma&1.44 [0.07]&1.72 [0.08]&&1.40 [0.08]&1.52 [0.08]\\
Oregon&1.23 [0.06]&1.29 [0.06]&&1.26 [0.08]&1.29 [0.08]\\
Pennsylvania&1.39 [0.09]&1.54 [0.09]&&1.40 [0.13]&1.46 [0.13]\\
Rhode Island&1.49 [0.08]&1.84 [0.10]&&1.38 [0.10]&1.52 [0.11]\\
South Carolina&1.44 [0.08]&1.70 [0.09]&&1.44 [0.09]&1.55 [0.09]\\
South Dakota&1.57 [0.08]&2.04 [0.11]&&1.38 [0.09]&1.59 [0.10]\\
Tennessee&1.49 [0.08]&1.83 [0.10]&&1.43 [0.09]&1.56 [0.09]\\
Texas&1.44 [0.10]&1.65 [0.10]&&1.53 [0.15]&1.62 [0.15]\\
Utah&1.52 [0.06]&1.86 [0.07]&&1.43 [0.09]&1.57 [0.09]\\
Vermont&1.21 [0.08]&1.25 [0.08]&&1.26 [0.15]&1.28 [0.15]\\
Virginia&1.33 [0.07]&1.45 [0.08]&&1.40 [0.11]&1.46 [0.11]\\
Washington&1.26 [0.07]&1.33 [0.07]&&1.30 [0.11]&1.34 [0.11]\\
West Virginia&1.35 [0.06]&1.50 [0.07]&&1.31 [0.07]&1.35 [0.07]\\
Wisconsin&1.49 [0.07]&1.77 [0.08]&&1.41 [0.08]&1.54 [0.09]\\
\bottomrule\end{tabular}
\end{footnotesize}
\begin{tablenotes}
\scriptsize
\item
Notes: Numbers in brackets are standard errors robust to serial correlation and cross-sectional correlation (robust2). The multiplication factor (MF) declines linearly from the high value to the low value.
\end{tablenotes}
\label{tab:state_R0_no_mit}
\end{table}
    
